COded Taking And Giving (COTAG): Enhancing Transport Layer Performance over Indoor Millimeter Wave Access Networks

Millimeter wave (mmWave) access networks have the potential to meet the high-throughput and low-latency needs of immersive applications. However, due to the highly directional nature of the mmWave beams and their susceptibility to beam misalignment and blockage resulting from user movements and rotations, the associated mmWave links are vulnerable to large channel fluctuations. These fluctuations result in disproportionately adverse effects on performance of transport layer protocols such as Transmission Control Protocol (TCP). To overcome this challenge, we propose a network layer solution, COded Taking And Giving (COTAG) scheme to sustain low-latency and high-throughput end-to-end TCP performance in dually connected networks. In particular, COTAG creates network encoded packets at the network gateway and each access point (AP) aiming to adaptively take the spare bandwidth on each link for transmission. Further, if one link bandwidth drops due to user movements, COTAG actively abandons the transmission opportunity by conditionally dropping packets. Consequently, COTAG actively adapts to link quality changes in mmWave access network and enhances the TCP performance without jeopardizing the latency of immersive content delivery. To evaluate the effectiveness of the proposed COTAG, we conduct experiments using off-the-shelf APs and network simulations. The evaluation results show that COTAG improves end-to-end TCP performance significantly on both throughput and latency.

==> sections/challenges.tex <==
% \documentclass[../main.tex]{subfiles}

% \begin{document}
\label{sec:challenges}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% change the fig topo into dual connectivity plus single connectivity.

% \subfile{TCP_BDP}
% TCP provides reliable, sequenced delivery of packets from a sender to a receiver. Although there are many different versions of TCP, they basically work as follows. A TCP sender sends a stream of packets to the TCP receiver. These packets travel from the sender to the receiver through the network, possibly experiencing different network effects including congestion, packet reordering, packet errors, packet losses, and wireless channel quality fluctuations. When a TCP receiver gets a packet, it sends back an acknowledgment to the TCP sender. According to the acknowledgement, the TCP sender controls its sending rate through adjusting the congestion window, which is the reflection of the bandwidth-delay product. 
% When TCP was first designed, the bandwidth-delay product of most networks were fairly small. 
% As bandwidth-delay product increased over time, primarily due to substantial increase in bandwidth, several modifications had to be made to the underlying protocol in order to make effective use of the network, i.e., maximize the sending rate without causing congestion and while maintaining a notion of fairness. 
% Despite these changes, TCP’s performance often falls well short of its potential in networks with large bandwidth-delay products. 
% This is especially so when the network includes a wireless link. 
% An intuitive explanation for this under performance is as follows.
% When acknowledgements reach the TCP sender, it makes two critical decisions: (i) whether a packet is lost in the network and (ii) whether the current sending rate is low or high relative to the network capacity. If a packet is deemed to be lost, the TCP sender retransmits the packet to assure reliable delivery. If the TCP sender deems that the network can support a higher sending rate, the TCP sender increases its sending rate. Otherwise, it reduces the sending rate. The goal of TCP is to keep the sending rate as high as possible without causing a congestion in the network. Each TCP sender also strives to share the network fairly with other contending TCP connections.

% In TCP parlance, at any given time, the available bandwidth is a measure of the maximum possible sending rate from the TCP sender to the receiver without causing a congestion in the network. The delay (or the round-trip time) is a measure of the time it takes for a packet to traverse the network from the TCP sender to the receiver and back to sender in the form of acknowledgement. Furthermore, the product of the bandwidth and the delay (often called the bandwidth-delay product of the network)  is measure of the maximum number of bits that can be “in transit” in the network between the TCP sender and the receiver, i.e., the maximum number of bits that can be sent by the TCP sender without yet receiving an acknowledgement for it.


% When TCP was first designed, the bandwidth-delay product of most networks were fairly small. As bandwidth-delay product increased over time, primarily due to substantial increase in bandwidth, several modifications had to be made to the underlying protocol in order to make effective use of the network, i.e., maximize the sending rate without causing congestion and while maintaining a notion of fairness. Despite these changes, TCP’s performance often falls well short of its potential in networks with large bandwidth-delay products. This is especially so when the network includes a wireless link. An intuitive explanation for this under performance is as follows.


% Since mmWave link can support high data rates comparable to those commonly available in the wired links, a network with mmWave link often has a large bandwidth. However, the data rate of a mmWave link fluctuates a lot. As stated earlier, the fluctuations are often caused by human movements, rotations and blockages. Since the wavelengths are in the millimeter range, movements in the order of the tens of millimeters may cause large fluctuations in the data rate. A simple illustrative example is as follows. A person wearing a AR/VR headset rotates their head while playing a game. 

% This disrupts the beam alignment between the transmit and receive antenna, which in turn causes the data rate to fall considerably until the underlying beam forming algorithms detect the issue and realign the beams. Meanwhile, the bits in transit from the TCP sender to the receiver experience severe congestion, which is sensed by the sender after a delay.

% For example, if the available bandwidth is 1 Gbps and the round-trip delay is 1 ms, then million bits are potentially in transit. When million bits experience congestion, TCP senders usually reduce the sending rate substantially. Meanwhile, the underlying beam forming algorithms may restore the alignment and the data rate becomes high again. However, the TCP sender cannot sense this increase. Instead, in order to preserve network fairness, it slowly strives to increase the sending rate. While the sending rate is slowly being increased, the end-to-end throughput is substantially below the available bandwidth. This process often repeats, and the TCP connection is often substantially below its full potential. Note that, if the bandwidth is small, the problem is not that acute because the sending rate may be able to catch up to the available bandwidth in relatively short amount of time.


% Although there are several potential solutions to this problem, it is very difficult to avoid the inherent delay for solutions at the transport layer to work effectively. In this paper, we argue that the network layer must address this issue. Our network layer solution assumes that the link and physical layers are also dealing the challenges posed by channel quality fluctuations in mmWave link. However, the inherent delays of detecting and dealing with the channel quality fluctuations \newadd{at} link and physical layers are large enough to adversely affect the performance at the transport layer (we show this through simulations later in the paper). Dual connectivity is another potential solution to this problem. An advantage of dual connectivity is that there will be no loss of connectivity unless both links are blocked simultaneously. As a result, at first glance, it appears that there is much greater chance of preserving transport layer performance. This optimism does not easily pan out because the transport layer such as TCP are not designed to handle the large numbers of out-of-sequence arrivals which may occur due to dual connectivity. In this paper, we use a technique called network coding (at the network layer) to combat the deleterious effects of channel quality fluctuations on transport layer performance.



% When TCP was first designed, the bandwidth-delay product of most networks were fairly small. 
% As bandwidth-delay product increased over time, primarily due to substantial increase in bandwidth, several modifications had to be made to the underlying protocol in order to make effective use of the network, i.e., maximize the sending rate without causing congestion and while maintaining a notion of fairness. 
% Despite these changes, TCP’s performance often falls well short of its potential in networks with large bandwidth-delay products.

While TCP provides reliable, sequenced delivery of packets from a sender to a receiver, TCP’s performance often falls well short of its potential in networks with large bandwidth-delay products.
This is especially so when the network includes a mmWave link. 
As stated earlier, while mmWave link can support high data rates, the data rate of a mmWave link fluctuates a lot due to human movements, rotations and blockages in AR/VR scenarios.
This human-induced interference disrupts the beam alignment between the transmit and receive antenna, which in turn causes the data rate to fall considerably until the underlying beam forming algorithms detect the issue and realign the beams. Meanwhile, the bits in transit from the TCP sender to the receiver experience severe congestion, which is sensed by the sender after a delay.
For example, if the available bandwidth is 1 Gbps and the round-trip delay is 1 ms, then million bits are potentially in transit. When million bits experience congestion, TCP senders usually reduce the sending rate substantially. Meanwhile, the underlying beam forming algorithms may restore the alignment and the data rate becomes high again. However, the TCP sender cannot sense this increase. Instead, in order to preserve network fairness, it slowly strives to increase the sending rate. While the sending rate is slowly being increased, the end-to-end throughput is substantially below the available bandwidth. 
% This process often repeats, and the TCP connection is often substantially below its full potential. 
% Note that, if the bandwidth is small, the problem is not that acute because the sending rate may be able to catch up to the available bandwidth in relatively short amount of time.


Although there are several potential solutions to this problem, it is very difficult to avoid the inherent delay for solutions at the transport layer to work effectively. In this paper, we argue that the network layer must address this issue. Our network layer solution assumes that the link and physical layers are also dealing the challenges posed by channel quality fluctuations in mmWave link. However, the inherent delays of detecting and dealing with the channel quality fluctuations at link and physical layers are large enough to adversely affect the performance at the transport layer (we show this through simulations later in the paper). Dual connectivity \ICC{with the assist of sub-6G} is another potential solution to this problem. An advantage of dual connectivity is that there will be no loss of connectivity unless both links are \ICC{broken} simultaneously, \ICC{which is unlikely to happen to sub-6G connection (assuming there is no contention)}. As a result, at first glance, it appears that there is much greater chance of preserving transport layer performance. This optimism does not easily pan out because the transport layer such as TCP are not designed to handle the large numbers of out-of-sequence arrivals which may occur due to \ICC{the fluctuating unbalance between mmWave and sub-6G link bandwidth in} dual connectivity. In this paper, we use a technique called network coding (at the network layer) to combat the deleterious effects of channel quality fluctuations on transport layer performance.
% As mentioned earlier, dual connectivity is one possible way of alleviating the challenges of channel fluctuations caused by human movements. An advantage of dual connectivity is that there will be no loss of connectivity unless both links are blocked simultaneously. As a result, at first glance, it appears that there is much greater chance of preserving AR/VR experience. This optimism does not easily pan out because the transport layer such as TCP are not designed to handle the large numbers of out-of-sequence  arrivals which may occur due to dual connectivity. 
% % Fig.~\ref{RealTCP} shows that dual connectivity can enhance the performance and mitigate the adversarial effect of fluctuations only when there is no latency. As latency increases, the transport layer performance degrades fairly rapidly. Shown in this figure, when the end-to-end propagation delay is zero, TCP throughput over dual connectivity is better than the single connectivity scenario. However, even as the propagation delay gets to 5ms, TCP-Cubic is not able to quickly recover from packet reordering effects and the throughput drops below that of single connectivity. 
% In this paper, we use a technique called network coding (at the network layer) to circumvent packet reordering issues.







%-----------------------%%%%%%%%----------------------%
% These challenges with mmWave links are illustrated through the following simulations. The scenarios of mmWave networks simulations are shown in Fig.~\ref{fig:topo}. This figure includes both single connectivity and dual connectivity scenarios with mmWave links. The left part in this figure describes single connectivity simulations. The single connectivity simulations are based on an indoor mmWave wireless access network with only one mmWave AP with modern beamforming techniques and the mobile device only connects with one beam on the AP to receive packets. As for dual connectivity, the simulations on the right part in this figure correspond to an indoor mmWave wireless access network formed by two mmWave APs with modern beamforming techniques. Each mmWave AP can form at least one beam to provide wireless connectivity to mobile devices. Moreover, each mobile device can associate with two separate beams to establish dual link connectivity and receive packets from both wireless links simultaneously. 

% %%%%%measurement of singel CH and dual CH
% In the simulation of dual connectivity, the channel quality fluctuations of the mmWave link are obtained from measurements in an experimental setup shown in Fig.~\ref{setup}.
% The mmWave link in the experimental setup is the connection between
% two commercially available IEEE 802.11ad supported wireless APs. In this figure, the receiving devices D1 and D2 associate with the mmWave APs AP1 and AP2 respectively. Since there is no commercially available mobile device which can associate two mmWave beams simultaneously, we use D1 and D2 together to represent the mobile device which acquires this functionality and we think this functionality is likely to be achieved in the mmWave networks. 
% In this setup, we put the receiving devices D1 and D2 at different locations to simulate the user movements in the AR/VR application such that he/she moves in the vicinity of the APs. As the user moves, the quality of both links changes concurrently, some times the data rates in both links are positively correlated and in other times they are negatively correlated. The trace of channel measurements from the experimental setup was input to the simulation run in network simulator NS-2 \cite{ns2} in the form of data rates. The simulation run also considers the effect of different packet error rate (PER) and network latency conditions. This experiment setup is also suitable for the simulation of single connectivity with a mmWave link. In this case, we only need to use one link in this setup.





% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.99\columnwidth]{images/sinndual.png}%\vspace{-3mm}
%   \caption{Illustration of the mmWave wireless access network.}%\vspace{-3mm}
%   \label{fig:topo}
% \end{figure}

% \begin{figure}[!h]
% \center{\includegraphics[width=0.8\columnwidth]{setup.png}}
% %\vspace{-10pt}
% \caption{\label{setup} Real mmWave channel measurement setup with APs and receiving devices.}
% %\vspace{-20pt}
% \end{figure}

% Fig.~\ref{ideal}, \ref{wiredvswireless}, \ref{RealTCP} show some of the challenges with
% mmWave links. They present results from simulation runs where an AR/VR application uses TCP to assure reliable, sequenced delivery of packets with the packet size of 128 bytes. The version of TCP is Cubic \cite{Ha2008}, which is specific designed for high throughput scenarios.
% Fig.~\ref{ideal} includes the performance of TCP over an actual wireless mmWave link with fluctuations and the performance of TCP over an ideal wireless mmWave link with stable bandwidth equal to the average bandwidth of the actual mmWave link. These two types of link are also assumed to have zero PER, so we only present the impact of fluctuations and latency in this figure. The comparison between the performance of TCP on an ideal mmWave link and on an actual mmWave link with zero PER shows that the channel quality fluctuations itself reduces the end-to-end throughput significantly. For instance, at a RTT delay of about 10ms, the TCP throughput over an actual mmWave link is about half of that of a equivalent ideal link, primarily due to link bandwidth fluctuations. On top of this, Fig.~\ref{wiredvswireless} presents the performance of TCP over an actual wireless mmWave link with different PER. Fig.~\ref{wiredvswireless} further shows that packet transmissions over wireless links are also susceptible to bit errors, resulting in unrecoverable packet losses/errors. These errors further decrease TCP throughput. For instance, at a RTT of 10ms, and a PER of 0.1\%, the end-to-end throughput is less than a third of the performance on mmWave link with zero PER. This adverse degradation in performance is the key problem we propose to address in this paper. 

% As mentioned earlier, dual connectivity is one possible way of alleviating the challenges of channel fluctuations caused by human movements. An advantage of dual connectivity is that there will be no loss of connectivity unless both links are blocked simultaneously. As a result, at first glance, it appears that there is much greater chance of preserving AR/VR experience. This optimism does not easily pan out because the transport layer such as TCP are not designed to handle the large numbers of out-of-sequence  arrivals which may occur due to dual connectivity. Fig.~\ref{RealTCP} shows that dual connectivity can enhance the performance and mitigate the adversarial effect of fluctuations only when there is no latency. As latency increases, the transport layer performance degrades fairly rapidly. Shown in this figure, when the end-to-end propagation delay is zero, TCP throughput over dual connectivity is better than the single connectivity scenario. However, even as the propagation delay gets to 5ms, TCP-Cubic is not able to quickly recover from packet reordering effects and the throughput drops below that of single connectivity. In this paper, we use a technique called network coding (at the network layer) to circumvent packet reordering issues.




% \begin{figure}[!h]
% \center{\includegraphics[width=0.9\columnwidth]{images/ideal.png}}
% %\vspace{-10pt}
% \caption{\label{ideal} The end-to-end throughput comparison between ideal and actual mmWave wireless links with different latency.}
% \vspace{-10pt}
% \end{figure}

% \begin{figure}[!h]
% \center{\includegraphics[width=0.9\columnwidth]{images/wireless.png}}
% %\vspace{-10pt}
% \caption{\label{wiredvswireless} The end-to-end throughput of actual mmWave wireless links with different packet error rates and latency.}
% \vspace{-10pt}
% \end{figure}



% \begin{figure}[!h]
%     \center{\includegraphics[width=1\columnwidth]{images/DualvsSin.png}}
% %\vspace{-10pt}
%     \caption{\label{RealTCP} The short-term throughput during immersive data bursts of TCP-CUBIC with different packet error rates and latency.}
%     \vspace{-10pt}
% \end{figure}

%-----------------------%%%%%%%%----------------------%


% COMMANDED FOR REVIEW\rr{The simulation compares the throughput
%between wired links and mmWave links with different latency
%and packet error rate (PER). \rg{The wired links and mmWave links have the same average bandwidth in this simulation.} In this figure, different figures
%correspond to the wired link and wireless links with different
%PER. For each curve, as its latency grows, the corresponding
%end-to-end TCP throughput decreases. The curves show that
%as the link changes from wired to wireless, the end-to-end
%throughput drops faster as the latency increases, and this is
%the same as PER increases on wireless links. These results
%indicates that the performance of mmWave links is severely
%vulnerable to unstable channel conditions and latency.}

% As mentioned earlier, dual connectivity is one possible way of alleviating the challenges of channel fluctuations caused by human movements. An advantage of dual connectivity is that there will be no loss of connectivity unless both links are blocked simultaneously. As a result, at first glance, it appears that there is much greater chance of preserving AR/VR experience. This optimism does not easily pan out because the transport layer such as TCP are not designed to handle the large numbers of out-of-sequence  arrivals which may occur due to dual connectivity. %COMMANDED FOR REVIEW\rr{This is illustrated in Fig.~\ref{RealTCP}. The simulations in this figure correspong to an indoor mmWave wireless access network formed by two mmWave access points (APs) with modern beamforming techniques. Each mmWave AP can form at least one beam to provide wireless connectivity to mobile devices. Moreover, each mobile device can associate with two separate beams to establish dual network connectivity can thus receive packets from both wireless links simultaneously. The data rates of the wireless links are taken from measurement setup shown in Fig.~\ref{setup}. In this setup, the user movements in the AR/VR application are such that he/she moves in the vicinity of the access points. As the user moves, the quality of both links change concurrently, some times the data rates in both links are positively correlated and in other times they are negatively correlated. The trace of channel measurements from the experimental setup was input to the simulation run in network simulator NS-2 \cite{ns2}. The simulation run also considers the effect of different PER and network latency conditions.}
% Fig.~\ref{RealTCP} shows that dual connectivity can enhance the performance and mitigate the adversarial effect of fluctuations only when there is no latency. As latency increases, the transport layer performance degrades fairly rapidly.

% Fig.~\ref{wiredvswireless} evaluates the impact of channel quality fluctuations of a mmWave link on the end-to-end TCP performance with single connectivity. For comparison, 
% Fig.~\ref{wiredvswireless} includes the performance of TCP over a wired link with bandwidth equal to the average bandwidth of the mmWave link. The wired link is also assumed to have zero PER. Comparing the performance of TCP on wired mmWave with zero PER shows that the channel quality fluctuations itself reduces the end-to-end throughput significantly. For instance, at a round trip time (RTT) delay of about 10ms, the TCP throughput over mmWave link is about half of that of a equivalent wired link, primarily due to link bandwidth fluctuations. 
% On top of this,  
% Fig.~\ref{wiredvswireless} shows some of the challenges with
% mmWave links. It presents results from a simulation run where
% an AR/VR application uses TCP to assure reliable, sequenced delivery of packets with
% the packet size of 128 bytes. The version of TCP is Cubic \cite{Ha2008}, which is specific designed for high throughput scenarios.
% The channel quality fluctuations of the mmWave link in the simulation run
% are obtained from measurements in an experimental setup shown in Fig.~\ref{fig:topo}.
% The mmWave link in the experimental setup is the connection between
% two commercially available IEEE 802.11ad supported wireless APs.
% \rb{This is illustrated in Fig.~\ref{RealTCP}. The simulations in this figure correspond to an indoor mmWave wireless access network formed by two mmWave APs with modern beamforming techniques. Each mmWave AP can form at least one beam to provide wireless connectivity to mobile devices. Moreover, each mobile device can associate with two separate beams to establish dual link connectivity and receive packets from both wireless links simultaneously. The data rates of the wireless links are taken from measurement setup shown in Fig.~\ref{setup}. In this setup, the user movements in the AR/VR application are such that he/she moves in the vicinity of the APs. As the user moves, the quality of both links changes concurrently, some times the data rates in both links are positively correlated and in other times they are negatively correlated. The trace of channel measurements from the experimental setup was input to the simulation run in network simulator NS-2 \cite{ns2}. The simulation run also considers the effect of different packet error rate (PER) and network latency conditions.}
%\rr{Human movements in and around the wireless setup is one of causes of the channel quality fluctuations.}
%/

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% As the mmWave band brings the channel capacity to a new high level, there are also challenges. One challenge with the mmWave band is that the beams are substantially more directional than the conventional sub-6 GHz band.
% Furthermore, link bandwidth degrades more severely at the mmWave band than at the sub-6 GHz band. 
% For example, the 60 GHz signal attenuates 15 to 20 dB
% for the first-order reflected path as compared to the line-of-sight (LOS) path. Although adaptive beam management can alleviate
% deterioration in channel conditions, detecting a change in the channel conditions as well as reforming the beams takes time.
% The delays incurred in adapting the beams adversely affect the end-to-end latency and the resulting end-to-end throughput, which in turn degrades AR/VR experience.
% Finally, at certain frequencies especially around the 60 GHz band, the mmWave channels are highly
% susceptible to human blockages. This is because there is a significant absorption up notch by water molecules
% and humans are mostly water. \rb{Fig.~\ref{wiredvswireless} shows the challenge with mmWave links in a simulation run. In the simulation run, an AR/VR application uses Transmission Control Protocol (TCP) to assure reliable, sequenced delivery of packets with the packet size of 128 bytes. The version of TCP is Cubic \cite{Ha2008}. The mmWave links are collected using commercial devices, and their fluctuations introduced by human movements are also considered. This simulation compares the throughput between wired links and mmWave links with different latency and packet error rate (PER). In this figure, different figures correspond to the wired link and wireless links with different PER. For each curve, as its latency grows, the corresponding end-to-end TCP throughput decreases. The curves show that as the link changes from wired to wireless, the end-to-end throughput drops faster as the latency increases, and this is the same as PER increases on wireless links. These results indicates that the performance of mmWave links is severely vulnerable to unstable channel conditions and latency.}



% Channel fluctuations caused by human movements and blockages may be alleviated either by waiting for the blockages
% to dissipate by human movement or by reforming the beams or by handing off the connection to  a different 
% access point. All of these ways of alleviating the channel degradation incur delays which are detrimental to AR/VR experience.
% One promising approach to avoid the delays is dual connectivity. In dual connectivity, the user is concurrently connected
% through two wireless links, either through two different access points or through the same access point but via different beams.
% As long as only one beam is blocked by human movement, contents can be delivered to the AR/VR application, albeit at a possibly
% reduced data rate. Since there will be no total loss of connectivity unless both links are blocked, there is potential to preserve
% AR/VR experience. And we pursue this approach in the paper. 

% For simplicity of presentation, we assume that the dual connectivity is over two mmWave beams for the connection between the user device and the gateway. As illustrated in Fig.~\ref{fig:topo}, we consider an indoor mmWave wireless access network formed by multiple mmWave access points (APs),
% and with modern beamforming techniques. Each mmWave AP can form at
% least one beam to provide wireless connectivity to mobile devices. We
% also assume that each mobile device can associate with two separate
% beams to establish dual network connectivity. 
% Note that, the two beams may be either from two mmWave APs or from
% a single mmWave AP. In either case, the mobile device can
% receive packets from both wireless links simultaneously. For example,
% in Fig.~\ref{fig:topo}, the mobile device at the left hand side
% has dual connectivity from two mmWave APs while that
% on the right hand side obtains dual connectivity from the same mmWave
% AP.  


% It is clearly possible to provide dual connectivity
% over different frequency bands, one over mmWave and the other over sub-6 GHz. Such dual-band, dual connectivity have to address the challenge of potentially wide difference in the data rates of the two links even when both links are not blocked. There are many papers in literature which focus on dual band, dual connectivity challenges \cite{Kibria2018, Polese2017_2}. In this paper, we focus on the scenario where the user is fortunate enough to have dual connectivity through different mmWave band. We anticipate that this will occur more in the future because the number of antennas in mmWave communication systems is growing rapidly and providing dual beam connectivity will not be a major issue.

% \rb{However, even purely dual connectivity can not fully overcome the challenge in maintaining high throughput in mmWave networks. This challenge is demonstrated in Fig.~\ref{RealTCP}. At the link layer of this simulation, the user is connected over two mmWave access points in dual connectivity and in single connectivity, the user is connected with only one mmWave access point. The data rates of the wireless links are taken from measurement setup shown in Fig.~\ref{setup}. In this setup, the user movements in the AR/VR application are such that he/she moves in the vicinity of the access points. As the user moves, the quality of both links change concurrently, some times the data rates in both links are positively correlated and in other times they are negatively correlated. The trace of channel measurements from the experimental setup was input to the simulation run in network simulator NS-2 \cite{ns2}. The simulation run also considers the effect of different PER and network latency conditions. Fig.~\ref{RealTCP} shows that dual connectivity can enhance the performance and mitigate the adversarial effect of fluctuations only when there is no latency. And \method\ in this paper is focused on the enhanced solution based on the use of dual connectivity.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% However, even with dual connectivity, maintaining high throughput is a challenge in mmWave networks. Addressing these challenges
% is the focus of this paper. Fig.~\ref{RealTCP} demonstrates this challenge. The figure shows results of a simulation run. In the simulation
% run, an AR/VR application uses Transmission Control Protocol (TCP) to assure reliable, sequenced delivery of packets. At the
% link layer, the user is connected over two mmWave access points. The version of TCP is Cubic \cite{Ha2008}. The data rates of the two
% wireless links are taken from measurement setup shown in Fig.~\ref{setup}. In this setup, the user movements in the AR/VR application
% are such that he/she moves in the vicinity of the access points. As the user moves, the quality of both links change concurrently,
% some times the data rates in both links are positively correlated and in other times they are negatively correlated. The trace
% of channel measurements from the experimental setup was input to a simulation run in network simulator NS-2 \cite{ns2}. The end-to-end
% TCP throughput was obtained from NS-2.  
